NAST: Noise Aware Speech Tokenization for Speech Language Models

Speech tokenization is the task of representing speech signals as a sequence of discrete units. Such representations can be later used for various downstream tasks including automatic speech recognition, text-to-speech, etc. More relevant to this study, such representation serves as the basis of Speech Language Models. In this work, we tackle the task of speech tokenization under the noisy setup and present NAST: Noise Aware Speech Tokenization for Speech Language Models. NAST is composed of three main components: (i) a predictor; (ii) a residual encoder; and (iii) a decoder. We evaluate the efficiency of NAST considering several spoken language modeling tasks and show that NAST is superior to the evaluated baselines across all setups. Lastly, we analyze NAST and show its disentanglement properties and robustness to signal variations in the form of noise, reverberation, pitch-shift, and time-stretch. Code and pre-trained models are available at https://github.com/ShovalMessica/NAST.

==> 03_back.tex <==
\section{Background}
\label{sec:back}
We operate under the GSLM framework. The typical GSLM pipeline incorporates three principal components: (i) Speech-to-unit conversion, also known as speech tokanization, (ii) Unit-based language modeling, and (iii) Unit-to-speech synthesis. Each component is developed independently. The process of speech reconstruction can bypass the language modeling stage by directly inputting the quantized units into the unit-to-speech synthesizer~\cite{polyak2021speech}. In this work, we focus on the speech tokanization part. 

\newpara{Speech-to-unit} conversion involves transforming the raw audio signals into a set of discrete tokens. This process usually begins with converting speech into a continuous latent space, followed by a quantization step to discretize these representations into a sequence of tokens~\cite{on_generative, polyak2021speech, popuri2022enhanced, lee2021direct, kharitonov2021text, kreuk2021textless, kharitonov2022textless, nguyen2022generative, borsos2022audiolm, tjandra2019vqvae, tjandra2020transformer}.

Formally, let $\mathcal{X} \subset \mathbb{R}$ represent the space of audio samples. A raw audio signal is a series of samples $x = (x_1,\ldots, x_T)$, where each $x_t\in\mathcal{X}$ for $1\leq t \leq T$. An encoding network, denoted as $f$, accepts a speech utterance as input and outputs a sequence of spectral features at a reduced sampling rate, $f(x) = (v_1, \dots, v_{T'})$. The structure of the encoder $f$ is not specified. Various encoders have been assessed, including Mel-spectrogram, Contrastive Predictive Coding (CPC)\cite{oord2018representation}, wav2vec2\cite{baevski2020wav2vec}, and HuBERT~\cite{hubert}, by \cite{on_generative}. The continuous features generated by these models are quantized into discrete tokens, $z = (z_1,\ldots,z_{T'})$, through k-means clustering. Each token $z_i$ is an integer within the set ${1,..,K}$ for $1\le i \le T'$, where $K$ is the total number of discrete tokens. The quantization process is represented by $E$.

\newpara{Unit Language Model} operates on the discrete unit sequences, $z$, extracted from the speech. This model is designed to learn the distribution of these unit sequences, enabling the direct modeling of speech without reliance on text. Such language models facilitate speech generation, both conditionally and unconditionally, mimicking early human language acquisition without written language knowledge. This approach also allows the capture of prosodic elements~\cite{kharitonov2021text}, speaker characteristics~\cite{borsos2022audiolm}, and natural conversational patterns~\cite{nguyen2022generative}, which are not encapsulated by textual data.

\newpara{Unit-to-speech} synthesis is the process of converting discrete speech units back into audible speech waveforms. Initially, \cite{on_generative} implemented a Tacotron 2.0-based framework with a WaveGlow vocoder~\cite{prenger2019waveglow} for this purpose. Subsequently, \cite{polyak2021speech} introduced a HiFi-GAN-based unit vocoder for direct unit-to-speech conversion, offering enhanced generation quality and efficiency by utilizing a single model. Further advancements by \cite{kreuk2021textless} and \cite{lee2021direct} have enriched unit-based vocoders with emotional and duration modeling capabilities for tasks such as speech emotion conversion and direct speech-to-speech translation, respectively.
